Analytic Evolution for Complex Coupled Tight-Binding Models: Applications to Quantum Light Manipulation

We present analytic solutions to the evolution in generalized tight-binding models, which consider complex first-neighbor couplings with equal amplitude and arbitrary phases. Our findings provide a powerful tool for efficiently calculating expectation values and correlations within the system, which are otherwise difficult to compute numerically. We apply our results to relevant examples in quantum light manipulation using N-port linear couplers, describing the evolution of single(multi)-mode squeezing, single photon added (subtracted) Gaussian states, and second-order site-to-site photon correlations. Significantly, our analytic results outperform standard numerical calculations. Our study paves the way for a comprehensive mathematical framework describing the spatial evolution of quantum states across a wide range of physical systems governed by the tight-binding model.

==> provisorio_metodos.tex <==
The associated evolution operator $U=\exp(-iHt/\hbar)$ relates the input and output annihilation operators by the set of transformations $a_m'=U^{-1}a_mU$. Using the BCH formula and the commutation relations  $[a_k,a_\ell^\dagger]=\delta_{k\ell}$ we obtain a matrix equation in the form of \eqref{eq:ap}, with  $A^{(N)}$ being a $N\times N$ matrix all of whose coefficients are found  to have the general form
%Para el caso abierto, encontramos que el corchete cuadrado de la ecuacion (7)
\begin{equation}\label{eq:A_mn}
 A^{(N)}_{m,n}=\exp(-i\phi_{m,n})\beta_{m,n}^{(N)}\,,
\end{equation}
with
\begin{equation}\label{eq:definiciones}
 \phi_{m,n}=\Delta_{m-1}-\Delta_{n-1}\,,\qquad \beta_{mn}=\sum_{k=0}^\infty F_k C^k\,.
\end{equation}
%el conteo de caminos de la ecuación \eqref{eq:expBCHc} en el caso abierto esta asociado a los numeros Z. Esto lo calculamos mediante teoria de grafos y de forma directa con la formula BCH
Thus, $\beta_{m,n}^{(N)}$ denotes the infinite sum of powers of the complex coupling amplitude $C$ with real weights $F_k$, while all the information about the complex phases of the coupling  coefficients is captured by $\phi_{m,n}$ and $\Delta_n=\delta_1+\delta_2+\cdots+\delta_n$. Coefficients $F_k$ form a sequence determined by the recursive relation \eqref{eq:recur}, which can be rewritten by decomposing the initial condition ${\bf S}_0^{(r)}$ on the eigenvectors $\lbrace{\bm \varphi}_j\rbrace$ of the recursion matrix $R$. This leads to the following expression for the $n$-th term in the sequence:
\begin{equation}\label{eq:Snb}
 S_n^{(r)}=\sum\limits_{j=1}^p\eta_{j,r}\varphi_j^n\,,
\end{equation}
where $\varphi_j$ is the $j$-th eigenvalue of $R$. This formalism reduces the problem to diagonalize the recursion matrix $R$, i.e. to find the roots $\varphi_j$ of its characteristic polynomial $P_N(x)$; aftwerwards we must find the coefficients $\eta_{j,r}$ that go into decomposition \eqref{eq:Snb}.  By identifying the polinomial families containing $P_N(x)$ we find that its roots are (see Appendix \ref{Appendix:Derivation}%TODO
)
\begin{equation}\label{eq:vphi}
 \varphi_j=2\cos\left(\frac{j\pi}{N+1}\right)\,,\qquad\quad j=1,\ldots,N\,.
\end{equation}

